Measuring Machine Learning Harms from Stereotypes Requires Understanding Who Is Harmed by Which Errors in What Ways

As machine learning applications proliferate, we need an understanding of their potential for harm. However, current fairness metrics are rarely grounded in human psychological experiences of harm. Drawing on the social psychology of stereotypes, we use a case study of gender stereotypes in image search to examine how people react to machine learning errors. First, we use survey studies to show that not all machine learning errors reflect stereotypes nor are equally harmful. Then, in experimental studies we randomly expose participants to stereotype-reinforcing, -violating, and -neutral machine learning errors. We find stereotype-reinforcing errors induce more experientially (i.e., subjectively) harmful experiences, while having minimal changes to cognitive beliefs, attitudes, or behaviors. This experiential harm impacts women more than men. However, certain stereotype-violating errors are more experientially harmful for men, potentially due to perceived threats to masculinity. We conclude that harm cannot be the sole guide in fairness mitigation, and propose a nuanced perspective depending on who is experiencing what harm and why.

==> supp_notseparate.tex <==

\todo{NOT UPDATED}
\section{Sample Size Justification}

Our sample size selection method is recorded on Open Science Framework and is done as follows: Study 1 we selected the number such that each COCO object was labeled by 10 participants from each gender; once we saw there was sufficient consensus from Study 1, for the first part of Study 4 where we labeled OpenImages objects, we selected the number such that each OpenImages object was labeled by 5 participants from each gender; Study 3a we had three stimulus conditions across two objects, so for this between-subjects study selected the number to have 50 participants from each gender for each object-condition setting; Study 3b we had three stimulus conditions across four objects, but this is a within-subjects study so each participant sees all possible scenarios, and thus we again selected the number to have 50 participants from each gender; Study 4 we had 40 objects and as our last study ended up having the budget to have around 37.5 participants per object.

\section{Additional Results from Study 1}

We show the results of harm annotation in the abstract on the y-axis of Fig.~\ref{fig:study1_sum} for the 13 objects marked as stereotypes. We see large variations within stereotypical objects for whether the association is perceived to be harmful when it is disconnected from a particular impact. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/study1_sum.png}
    \caption{\textbf{Study 1 Results.} Participant responses for 80 objects in COCO dataset. The x-axis indicates the percentage of participants who indicated an object is a stereotype, where negative numbers indicate it is a stereotype about men, and positive numbers about women. For objects where more than half of the respondents indicate it is a stereotype, the y-axis indicates the percentage who marked it to be harmful.}
    \label{fig:study1_sum}
\end{figure}

\section{Additional Results from Study 2}

Here we present the full analyses we perform on the open-ended responses we received in Study 2 regarding why participants believe an object is a stereotype, and if so, why they find it harmful or not.

Our categorization for why an object is a stereotype or not are as follows (some responses did not fall into any of the categories):
\begin{itemize}
    \item Descriptive (45\%), e.g., for handbag and women: ``women are often seen wearing handbags and buying them''
    \item Occupation/role (22\%), e.g., for oven and women: ``Women are stereotyped to always be in the kitchen cooking while the men go out and work''
    \item Trait (11\%), e.g., for chair and men: ``sometimes men would be seen as coming home and just being lazy and lounging in their chair''
    \item Pop culture (8\%), e.g., for cow and women: ``Most people who describe a women as a cow are being harmful and hurtful''
    \item Connection to another object (5\%), e.g., for vase and women: ``I think women are seen as liking flowers, which are often put into a vase''
    \item Prescriptive (3\%), e.g., for handbag and women: ``society generally believes that only women should carry handbags''
\end{itemize}

Our categorization for why a stereotypical object is harmful is as follows (some responses did not fall into any of the categories):
\begin{itemize}
    \item Proscriptive, i.e., excluding (40\%), e.g., for dining table and women: ``it makes it looked down upon if a man cooks dinner.''
    \item Prescriptive, i.e., restricting (26\%), e.g., for dining table and women: ``I think it puts women in a box that says they must prepare dinner''
    \item Negative Trait (13\%), e.g., for handbag and women: ``It is harmful because it implies that women cares more about looks and their appearance.''
    \item Demeans (10\%), e.g., for cow and women: ``cow is a typical insult for a women a man doesn't like  (`stupid cow')''
    \item Objectifies (5\%), e.g., for cup and women: ``It is harmful because a cup is an object and it's comparing it to a woman''
    \item Sexism (3\%), e.g., for sandwich and women: ``make me a sandwich meme sexism''
    \item Incorrect (3\%), e.g., for sandwich and women: ``It's an old, tired stereotype that holds no merit.''
\end{itemize}

The following are the two reasons respondents listed a stereotype to not be harmful: not negative (96\%), e.g., for tie and men: ``I don't think it's harmful because it's just a fashion choice''; positive stereotype (4\%), e.g., for cake and women: ``cake can be used to describe a woman as sweet and nice looking. For that reason I don't find it harmful.''


\section{Behavior Caption Analysis from Study 3a}
% Here we explain in further detail our results from Study 2a. From 

% include the results of the 10 quantitative indices of our 11 total measures of pragmatic harms. Fig.~\ref{fig:pragmatic} shows these results for the stereotype-reinforcing error relative to the two controls of stereotype-neutral and stereotype-violating errors.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\textwidth]{Figures/pragmatic_both.png}
%     \caption{\textbf{Study 2a results.} The effect sizes and 95\% confidence intervals are reported for 10 of our 11 measures of pragmatic harm (for the behavior measure of captioning, we provide a descriptive analysis). Deviations from zero indicate that exposure to the stereotype-reinforcing stimulus resulted in a behavior, cognitive, or attitude change compared to exposure to the control condition. After correcting for the p-values using the Benjamini-Hochberg Procedure~\cite{benjamini2995falsediscovery}, we see no statistically significant effects.}
%     \label{fig:pragmatic}
% \end{figure}
Here we present an exploratory analysis of the captions produced by participants for the behavior task in Study 3a.
In Tbl.~\ref{tbl:caption} we compare the captions generated by participants across conditions, and find no statistically significant results.

% Overall, we find no evidence of pragmatic harms as a result of stereotype-reinforcing errors.

\begin{table}
\caption{Descriptive statistics about the captions annotated as a part of Study 3a's behavior measure for the stereotype of women and hair dryer, where toothbrush serves as the control neutral object.}
\label{tbl:caption}
% \begin{center}
% { |>{\centering\arraybackslash}p{1.4cm}|>{\centering\arraybackslash}p{1.4cm}|>{\centering\arraybackslash}p{.9cm}|>{\centering\arraybackslash}p{.9cm}|>{\centering\arraybackslash}p{.9cm}|} 

\begin{tabular}{|>{\centering\arraybackslash}p{2.3cm}|>{\centering\arraybackslash}p{2.2cm}|>{\centering\arraybackslash}p{2.2cm}|>{\centering\arraybackslash}p{1.0cm}|>{\centering\arraybackslash}p{1.0cm}|>{\centering\arraybackslash}p{1.0cm}|>{\centering\arraybackslash}p{1.0cm}|}
    \hline
    \multirow{2}{*}{Condition} &
      \multicolumn{2}{>{\centering\arraybackslash}p{4.4cm}|}{Mention of Hair Dryer / 
      
      Mention of Toothbrush} &
      \multicolumn{2}{>{\centering\arraybackslash}p{2.0cm}|}{Warmth} &
      \multicolumn{2}{>{\centering\arraybackslash}p{2.0cm}|}{Competence} \\ \hline
    Gender of Person Being Described & Women & Men & Women & Men & Women & Men \\
    \hline
    Stereotype-reinforcing &  1.095 (0.679-1.800) & 1.125 (0.679-1.800) & 6.750 $\pm$ 0.386 & 1.107 $\pm$ 0.327 & 1.222 $\pm$ 0.263 & 0.933 $\pm$ 0.225\\
    \hline
    Stereotype-violating & .810 (0.458-1.286) & .857 (0.222-2.500) & 1.182 $\pm$ 0.417 & 0.905 $\pm$ 0.384 & 0.632 $\pm$ 0.265 & 0.750 $\pm$ 0.248\\
    \hline
    Neutral & 0.913 (0.562-1.450) & 0.571 (0.100-1.750) & 1.300 $\pm$ 0.425 & 0.769 $\pm$ 0.300 & 0.783 $\pm$ 0.293 & 1.182 $\pm$ 0.229 \\
    \hline
  \end{tabular}
% \end{center}
\end{table}

\section{Additional Results from Study 3b}
For Study 3b not only did we ask for personal experiential harm from an error, but also societal harm, so that even if the participant does not personally feel harmed, they may feel it on behalf of the stereotyped group. There is a high correlation between the responses to these two versions of the question for each error, which is why we only reported results from personal harm in the main text.

We regress on harm value with the independent variables of stereotype condition, personal harm compared to societal harm, and their interaction effect.
We find that for stereotype-reinforcing vs neutral errors, the coefficient for personal or societal harm is $b = .22$ (95\% $CI$ [-.07, .51], $p=.143$), and that for the interaction effect to be $b = -.18$ (95\% $CI$ [-.59, .23], $p=.398$). For stereotype-reinforcing vs stereotype-violating errors, the coefficient for personal or societal harm is $b = .26$ (95\% $CI$ [-.03, .55], $p=.076$), and that for the interaction effect to be $b=-.22$ (95\% $CI$ [-.63, .19], $p=.288$). In other words, there is no statistically significant difference in the results for societal harm compared to personal harm.

% In our results, we were somewhat surprised to find that participants who identified as men did not even think stereotype-reinforcing errors would be more harmful towards society than those which are not, but this also follows from prior work which has found that algorithmic discrimination (as opposed to human discrimination) tends not to lead to moral outrage, which as an unfortunate consequence of not associating intent with machine learning errors, and often leads to a lack of collective action against such harms~\cite{bigman2022outrage}.




\section{Object Selection from OpenImages}
In OpenImages, of the 600 objects, we select the 20 marked with the most agreement to be stereotypically associated with men, and the 20 marked with the most agreement to be stereotypically associated with women. We then randomly select amongst 20 objects that are marked to have no gender stereotypes associated with them. Left out of this are all human-related categories: \textit{boy}, \textit{girl}, \textit{human eye}, \textit{human face}, \textit{human body}, \textit{human ear}, \textit{human arm}, \textit{human board}, \textit{human hand}; as well as \textit{invertebrate} because there was confusion amongst pilot testers about what this word meant.

The 20 objects stereotyped about men are: \textit{football helmet}, \textit{football}, \textit{cowboy hat}, \textit{hammer}, \textit{sports equipment}, \textit{jet ski}, \textit{truck}, \textit{tie}, \textit{golf ball}, \textit{beer}, \textit{skateboard}, \textit{briefcase}, \textit{plumbing fixture}, \textit{tire}, \textit{wrench}, \textit{suit}, \textit{missile}, \textit{tool}, \textit{rifle}, \textit{shotgun}. The 4 that we consider ``clothing,'' i.e., able to be worn, are \textit{football helmet}, \textit{cowboy hat}, \textit{tie}, \textit{suit}.

The 20 objects stereotyped about women are: \textit{ladybug}, \textit{doll}, \textit{hair spray}, \textit{lily}, \textit{hair dryer}, \textit{perfume}, \textit{kitchenware}, \textit{cat}, \textit{wine glass}, \textit{fashion accessory}, \textit{necklace}, \textit{flower}, \textit{handbag}, \textit{lipstick}, \textit{bathtub}, \textit{face powder}, \textit{cosmetics}, \textit{rose}, \textit{oven}, \textit{brassiere}. The 9 that we consider ``clothing,'' i.e., able to be worn, are \textit{necklace}, \textit{face powder}, \textit{fashion accessory}, \textit{lipstick}, \textit{brassiere}, \textit{cosmetics}, \textit{hair spray}, \textit{handbag}, \textit{perfume}.

The 20 neutral objects are: \textit{pillow}, \textit{owl}, \textit{giraffe}, \textit{balloon}, \textit{jellyfish}, \textit{stop sign}, \textit{french fries}, \textit{eraser}, \textit{shower}, \textit{orange}, \textit{chopsticks}, \textit{window}, \textit{personal flotation device}, \textit{bed}, \textit{goldfish}, \textit{zebra}, \textit{raccoon}, \textit{sea lion}, \textit{microphone}, \textit{popcorn}.

\section{Bias Amplification}
Bias amplification is a statistical notion that rests on the idea that any amplification of an existing bias is undesirable, and often used to implicitly capture stereotypes~\cite{zhao2017men, wang2021biasamp, wang2019balanced, hall2022biasamp}.
In this line of work, a ``bias'' is measured in the dataset, e.g., that women are correlated with object A, and so any amplification of this in the model's test-time predictions is considered undesirable, and likely the application of something like a stereotype. This ``bias'' is determined statistically, and two possible formulations come from \citet{zhao2017men} (Bias Amp) and \citet{wang2021biasamp} (Directional Bias Amp).
As an example, \citet{zhao2017men} measures oven, wine glass, and potted plant, to all be biased towards men. From our human annotations, we find all these of these objects to be biased towards women. Thus, mitigation algorithms directed at reducing either of these formulations of bias amplification would actually likely \textit{increase} certain types of harmful errors in an attempt to reduce overall bias amplification.
This formulation also assumes that every label is biased in a way such that one direction of error is worse than another, missing that many labels can be neutral in certain respects, e.g., bowl and table. 


We quantify two aspects of each bias amplification metric, which are its abilities to identify either objects as stereotypes (measured by calculating the percentage overlap between the top-$n$ ``biased'' objects and $n$ stereotypes) or the gender direction of the stereotype's alignment (measured by calculating the gender direction on the $n$ stereotyped objects). In Tbl.~\ref{tbl:biasamp} we can see that while both bias amplification metrics are able to approximate the gender that a stereotyped object is correlated with in the COCO dataset reasonably well, this is not true for identifying which objects are stereotypes, nor the gender alignment in the larger OpenImages dataset. Thus, attempts to reduce either metric of bias amplification are likely to inadvertently increase the number of stereotypical errors in an attempt to reduce a ``bias amplification'' error that may not actually be stereotypically harmful.

\begin{table}
\caption{Comparison of how correlated to human perceptions prior measures of bias amplification, which approximate the directions of bias that are more harmful, are.}
\label{tbl:biasamp}
% \begin{center}
% \begin{tabular}{ |>{\centering\arraybackslash}p{1.8cm}|>{\centering\arraybackslash}p{3.5cm}|>{\centering\arraybackslash}p{2.cm}|>{\centering\arraybackslash}p{2.cm}|>{\centering\arraybackslash}p{2.cm}| } 
\begin{tabular}{ >{\centering\arraybackslash}p{1.8cm} >{\centering\arraybackslash}p{3.5cm} >{\centering\arraybackslash}p{2.cm} >{\centering\arraybackslash}p{2.cm} >{\centering\arraybackslash}p{2.cm} } 
 \hline
Dataset & Metric & Pearson R & Identification of Stereotypes & Alignment of Stereotypes\\
\hline 
COCO & Bias Amp~\cite{zhao2017men} & .5722 & 7/13 (54\%) & 10/13 (77\%) \\
\cmidrule{2-5}
& Directional Bias Amp~\cite{wang2021biasamp} & .6507 & 6/13 (46\%) & 13/13 (100\%) \\
\hline
OpenImages & Bias Amp & .3912 & 124/249 (50\%) & 141/249 (57\%) \\
\cmidrule{2-5}
& Directional Bias Amp & .1502 & 120/249 (48\%) & 153/249 (61\%)\\
\hline
\end{tabular}
% \end{center}
\end{table}

\section{Automatic Discovery of Stereotypes}
Evaluation is sometimes considered secondary to algorithm development, and thus rapid and fully-automated evaluations are often prioritized over those requiring human input. Thus, one might imagine trying to 
% retain a human-free quality during evaluation and attempting to 
automate the determination of which labels are stereotypes, rather than soliciting judgments from human annotators.
% One attempt to implement our finding that stereotype-related errors are more harmful than neutral ones which retains the human-free nature of many existing fairness metrics could be automating the determination of which prediction targets are stereotypes, rather than soliciting opinions from human annotators.
% Given our findings, one could imagine a potential rebut to the notion that humans need to be incorporated into fairness evaluation of this form. This might take the shape of an argument that the human prior of stipulating errors which are aligned with stereotypes to be more harmful is sufficient human involvement. And, perhaps, rather than soliciting human involvement on which labels constitute a stereotype, a machine learning model could be leveraged to predict which of the objects are stereotypes. 
To test the limits of this approach, we train a variety of models (Support Vector Machine, Random Forest, and Multi-Layer Perceptron) with hyperparameter search over the number of features and find the highest ROC AUC for predicting whether an OpenImages object is a stereotype given an input of BERT word embeddings~\cite{devlin2019bert} to be 74\%. 
Erroneous predictions include \texttt{carnivore} (is stereotype), \texttt{tennis ball} (is not stereotype), \texttt{infant bed} (is stereotype), \texttt{soap dispenser} (is not stereotype), \texttt{handbag} (is stereotype). 
Given that an object is a stereotype, the highest ROC AUC at predicting which gender is being stereotyped is 85\%. 
Erroneous predictions include \texttt{mixer} (stereotyped with women), \texttt{doughnut} (stereotyped with men), \texttt{houseplant} (stereotyped with women), \texttt{wheel} (stereotyped with men).
These inadequate performance rates indicate that stereotypes are highly contextual, and even with the use of powerful word embeddings which capture bias and social context~\cite{garg2018quantify}, they are insufficient without human input. As we note in the main text, even if the growing power of large language models enables us to predict with higher accuracy which objects are stereotypes, we likely still may want to ensure these annotations come from people themselves~\cite{argyle2023many, hamalainen2023synthetic}, thus allowing room for positionality, explanation, and critical reflection.
% so they can explain the reasoning and logic behind their beliefs, e.g., to understand whether their feelings are based in justifiable concerns or bigotry.
% , we have strong reason to believe

\section{Connection to Open-Ended ML Tasks without Correctness}
We scoped our work to machine learning tasks which have a clear notion of error, i.e., ground-truth labels. Here, we consider the implications of our findings for other machine learning tasks which do not have such a clear notion of a error, for example in text generation.
We can also consider the implications of our findings for other machine learning tasks which do not have such a clear notion of a error, for example in text generation. 
% \citet{bolukbasi2016embeddings} and \citet{caliskan2017semantics} first brought to light that word embeddings mirror stereotypes in our society, such as about occupations and attributes from the Implicit Association Test~\cite{greenwald1998iat}. \citet{garg2018quantify} continue this thread of work on how word embeddings reflect societal stereotypes by using the shifting of word embedding biases over time to track societal stereotype changes.
Prior work brought to light that word embeddings mirror stereotypes in our society~\cite{bolukbasi2016embeddings, caliskan2017semantics}, such as about occupations and attributes from the Implicit Association Test~\cite{greenwald1998iat}. 
% It has also been shown that word embeddings reflect societal stereotypes by using the shifting of word embedding biases over time to track societal stereotype changes~\cite{garg2018quantify}.
% Notably, these works both represent a reflection of stereotypes in society within word embeddings, something even more explicitly done by \citet{garg2018quantify} who uses the shifting of biases in word embeddings over time to track stereotype changes in society. 
% However, these works do not provide much insight as to what that means for our use of these word embeddings, and potential feedback loop effects for their implications for society.
Since then, most follow-up work in this space seeks to remove nearly all gendered associations in text, conflating each such association with harmful ``bias.''
% In the follow-up work in this space 
Again we see a similar pattern to the logical fallacy of the harm of one type of error, e.g., a correlation of some set of stereotypical occupations to gender, extending to \textit{all} errors. The nuance is lost when gendered associations of all kinds in word embeddings are equated to stereotypes, and most notions of gender are targeted to be removed from the embeddings. To put this into perspective, in the large body of literature that has followed the discovery of gender biases in the embedding space~\cite{shin2020neutralizing, zhao2018gnglove, karve2019conceptor, dev2019vector, kaneko2019debiasing, ravfogel2020null, dev2020embeddings, manzini2019multiclass}, all eight of these works would, as far as we can tell, attempt just as much to debias words like ``table'' and ``apple'' as they would ``homemaker'' and ``doll.'' While it is not clear what exactly is the desired state of debiasing (e.g., describing the world as it is, prescribing the world as it ought to be, aligning with people's existing stereotypic expectations~\cite{wang2021acceptance}) it surely seems that more thinking should be done on the different implications of debiasing stereotypes as opposed to debiasing more neutral concepts.


